Partially Observable Stochastic Games with Neural Perception Mechanisms

Stochastic games are a well established model for multi-agent sequential decision making under uncertainty. In practical applications, though, agents often have only partial observability of their environment. Furthermore, agents increasingly perceive their environment using data-driven approaches such as neural networks trained on continuous data. We propose the model of neuro-symbolic partially-observable stochastic games (NS-POSGs), a variant of continuous-space concurrent stochastic games that explicitly incorporates neural perception mechanisms. We focus on a one-sided setting with a partially-informed agent using discrete, data-driven observations and another, fully-informed agent. We present a new method, called one-sided NS-HSVI, for approximate solution of one-sided NS-POSGs, which exploits the piecewise constant structure of the model. Using neural network pre-image analysis to construct finite polyhedral representations and particle-based representations for beliefs, we implement our approach and illustrate its practical applicability to the analysis of pedestrian-vehicle and pursuit-evasion scenarios.

==> strategy.tex <==
\section{Strategy synthesis}

This section dicusses how to synthesize strategies for the players based on the generated lower and upper bound functions.


\begin{algorithm}[tb]
\caption{Strategy of $\agent_1$ via lower bound}
\label{alg:strategy-agent-1}
\textbf{Input}: initial belief $(s_{1}^{\mathit{init}}, b_{1}^{\mathit{init}})$, PWC $\alpha$-functions $\Gamma$
\begin{algorithmic}[1] %[1] enables line numbers
\State $\alpha^{\mathit{init}} \leftarrow \arg\max_{\alpha \in \Gamma} \langle \alpha, (s_{1}^{\mathit{init}}, b_{1}^{\mathit{init}}) \rangle$
\State $\mathit{Act}((s_{1}^{\mathit{init}}, b_{1}^{\mathit{init}}), \alpha^{\mathit{init}})$
\Function{$\mathit{Act}$}{$(s_1, b_1),  \alpha $}
\State $(u_1^{\star}, \hat{\lambda}^{\star}, \hat{V}^{\star}) \leftarrow$ solution to LP \eqref{eq:LP-minimax} at $(s_1, b_1)$ subject to $\overline{\alpha}^{\star} \ge \alpha$
\State $u_2^{\star} \leftarrow $ $\agent_2$'s assumed strategy in $[TV_{\mathit{LB}}^{\Gamma}](s_1, b_1)$ under $u_1^{\star}$ via \lemaref{lema:equilibrium-strategy-lower}
\State sample and play $a_1 \sim u_1^{\star}$
\State $s_1' \leftarrow$ observed $\agent_1$'s agent state
\State $\mathit{Act}((s_1', b_1^{s_1, a_1, u_2^{\star}, s_1'}), \hat{\alpha}^{\star a_1, s_1'})$
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[tb]
\caption{Strategy of $\agent_2$ via upper bound}
\label{alg:strategy-agent-2}
\textbf{Input}: initial belief $(s_{1}^{\mathit{init}}, b_{1}^{\mathit{init}})$, belief-value set $\Upsilon = \{ ((s_1^k, b_1^k), y_k) \mid k \in I\}$
\begin{algorithmic}[1] %[1] enables line numbers
\State $\mathit{Act}(s_{1}^{\mathit{init}}, b_{1}^{\mathit{init}})$
\Function{$\mathit{Act}$}{$s_1, b_1$}
\State $(u_2^{\star}, \hat{\lambda}^{\star},  \hat{V}^{\star}, \hat{c}^{\star}, V^{\star}) \leftarrow$ solution to LP \eqref{eq:LP-minimax-upper} at $(s_1, b_1)$
\State $(s_1, s_E) \leftarrow$ current observed state
\State sample and play $a_2 \sim u_2^{\star}(\cdot \mid s_1, s_E)$
\State $(a_1, s_1') \leftarrow $ $\agent_1$'s action and updated agent state
\State $\mathit{Act}(s_1', b_1^{s_1, a_1, u_2^{\star}, s_1'})$
\EndFunction
\end{algorithmic}
\end{algorithm}
